On The Quality Of Cryptocurrency Markets: Centralized Versus Decentralized Exchanges

We analyze the market quality of centralized crypto exchanges (CEXs) and decentralized blockchain-based venues (DEXs) using a unique and comprehensive dataset. Focusing on two fundamental aspects, transaction costs and deviations from the no-arbitrage condition, we estimate the causal effect of ``gas fees'' on DEX market quality. We show that these fixed costs impose a significant burden on relatively small trades and cause persistent arbitrage deviations. Conversely, DEXs offer more competitive transaction costs for larger trades, offering a more favorable environment for institutional investors. Furthermore, we provide causal evidence that innovations aimed at enhancing the flexibility of liquidity provision in DEX markets lead to sizeable improvements in market quality.

==> TAB/AMM_AB_table_SC.tex <==
\begin{tabular}{rrrrrrrrr}
\toprule
   &     &    &  &                   
                            $\qquad\,$USDC &  $\qquad\,$USDC &  $\qquad\,$USDT &  $\qquad\,$LINK &  $\qquad\,$USDC \\
   &     &    &  &                  USDT &          BTC &           BTC &           USDT &          USDT \\
   Fees & Liq & Gas & $\Delta V$ &  ETH &           ETH &           ETH &            ETH &          BTC \\
\midrule
\multicolumn{9}{c}{\textbf{Panel A: Current gas prices}}\\
\midrule
   30 &    1 &    1 &        1 &          122.03 &          189.01 &          959.83 &          785.41 &          967.91 \\
   10 &    1 &    1 &        3 &           62.38 &          129.55 &          902.72 &          727.76 &          910.70 \\
    5 &    1 &    1 &        6 &           47.43 &          114.65 &          888.40 &          713.31 &          896.36 \\
   30 &   10 &    1 &       10 &          100.54 &          121.19 &          371.67 &          313.02 &          374.25 \\
   10 &   10 &    1 &       30 &           40.96 &           61.53 &          312.76 &          253.93 &          315.34 \\   
\midrule
\multicolumn{9}{c}{\textbf{Panel B: Lower gas prices}}\\
\midrule
   30 &    1 &  500 &        1 &           91.18 &           94.18 &          129.98 &          121.49 &          130.35 \\
   10 &    1 &  500 &        3 &           31.42 &           34.44 &           70.34 &           61.83 &           70.71 \\
    5 &    1 &  500 &        6 &           16.44 &           19.46 &           55.40 &           46.87 &           55.76 \\
   30 &   10 &  500 &       10 &           90.22 &           91.14 &          102.47 &           99.78 &          102.59 \\
   10 &   10 &  500 &       30 &           30.45 &           31.38 &           42.75 &           40.05 &           42.87 \\
\\[-0.8em]     
\bottomrule
\end{tabular}


==> TAB/AMM_TC_4_SC.tex <==
\begin{tabular}{rrrrrrrrr}
\toprule
 &  &   & &                          $\,\qquad$BTC &  $\,\qquad$ETH  &  $\,\qquad$ LINK &  $\,\qquad$USDC &  $\,\qquad$USDC \\
 Fees &  Liq &  Gas &  $\Delta V$ &  $\,\qquad$ETH &  $\,\qquad$USDT &  $\,\qquad$ ETH  &  $\,\qquad$ETH  &  $\,\qquad$USDT \\
\midrule
\multicolumn{9}{c}{\textbf{Panel A: Current gas prices}}\\
\midrule
    30 &    1 &    1 &        1 &    57.75 &    57.64 &     59.74 &     57.49 &      60.18 \\
    10 &    1 &    1 &        3 &    37.75 &    37.64 &     39.75 &     37.49 &      40.19 \\
     5 &    1 &    1 &        6 &    32.75 &    32.65 &     34.75 &     32.49 &      35.19 \\
    30 &   10 &    1 &       10 &    56.82 &    56.81 &     57.02 &     56.79 &      57.06 \\
    10 &   10 &    1 &       30 &    36.82 &    36.81 &     37.02 &     36.80 &      37.06 \\
\midrule
\multicolumn{9}{c}{\textbf{Panel B: Lower gas prices}}\\
\midrule
    30 &    1 &  500 &        1 &    31.09 &    30.98 &     33.08 &     30.83 &      33.52 \\
    10 &    1 &  500 &        3 &    11.09 &    10.98 &     13.09 &     10.83 &      13.53 \\ 
     5 &    1 &  500 &        6 &     6.09 &     5.98 &      8.09 &      5.83 &       8.53 \\
    30 &   10 &  500 &       10 &    30.16 &    30.15 &     30.36 &     30.13 &      30.40 \\
    10 &   10 &  500 &       30 &    10.16 &    10.15 &     10.36 &     10.13 &      10.40 \\   
\bottomrule
\end{tabular}


==> TAB/FTX_DD_NB.tex <==
\begin{tabular}{lcccc}
\toprule
                 & (1)       & (2)       & (3)        & (4)        \\
\midrule
 Dep. Variable   & volume    & volume    & log_volume & log_volume \\
 DEX $	imes$ FTX & 1.100***  & 1.100***  & 0.303***   & 0.303***   \\
                 & (3.564)   & (3.572)   & (3.532)    & (3.540)    \\
 DEX             & -3.410*** & -3.410*** & -1.439***  & -1.439***  \\
                 & (-12.733) & (-12.760) & (-22.522)  & (-22.569)  \\
 FTX             & -1.100*** & -1.326*** & -0.303***  & -0.333***  \\
                 & (-3.564)  & (-8.613)  & (-3.532)   & (-7.778)   \\
 Intercept       & 3.410***  &           & 1.439***   &            \\
                 & (12.733)  &           & (22.522)   &            \\
 Observations    & 242       & 242       & 242        & 242        \\
 R-squared       & 0.696     & 0.713     & 0.896      & 0.905      \\
 Month FE        &           & Yes       &            & Yes        \\
SEs clustering: & Time & Time & Time & Time \\
\bottomrule
\end{tabular}


==> TAB/NFT_first_stage.tex <==
\begin{tabular}{lccc}
\toprule
                 & (1)              & (2)              & (3)              \\
\midrule
 Dep. Variable   & Median Gas Price & Median Gas Price & Median Gas Price \\[1em]
 NFT Mint Volume & 5.873***         & 6.192***         & 6.208***         \\
                 & (5.792)          & (4.023)          & (4.036)          \\[1em]
 ETH_abs_ret     &                  &                  & 3.549***         \\
                 &                  &                  & (7.704)          \\[1em]
 Intercept       & -9.685           &                  &                  \\
                 & (-0.885)         &                  &                  \\[1em]
 Observations    & 14,878           & 14,878           & 14,878           \\
 R-squared       & 0.014            & 0.437            & 0.439            \\
 Time FEs        &                  & Yes              & Yes              \\
\bottomrule
\end{tabular}


==> TAB/TC_reg.tex <==
\begin{tabular}{lccccccccc}
\toprule
{}                      & (1)          & (2)          & (3)          & (4)             & (5)          & (6)          & (7)          & (8)             & (9) \\
\midrule
Dep. Variable           & CEX    & CEX    & CEX    & CEX    & DEX    & DEX    & DEX    & DEX    & DEX - CEX \\
                      & TCs    & TCs    & TCs    & TCs    & TCs    & TCs    & TCs    & TCs    & TCs \\
&  &  &  &  &  &  &  & & \\
Lagged CEX TC           & 0.810***     &              &              &                 &              &              &              &                 &                 \\
                        & (15.128)     &              &              &                 &              &              &              &                 &                 \\[1.1em]
Lagged DEX TC           &              &              &              &                 & 0.808***     &              &              &                 &                 \\
                        &              &              &              &                 & (8.185)      &              &              &                 &                 \\[1.1em]
Average CEX TCs         &              & 1.015***     &              &                 &              & 2.287***     &              &                 &                 \\
                        &              & (21.249)     &              &                 &              & (21.670)     &              &                 &                 \\[1.1em]
Average DEX TCs         &              &              & 0.376***     &                 &              &              & 1.001***     &                 &                 \\
                        &              &              & (22.065)     &                 &              &              & (95.879)     &                 &                 \\[1.1em]
ETH Volume in USD       &              &              &              & 0.068           &              &              &              & 0.608***        & 0.472***        \\
                        &              &              &              & (1.123)         &              &              &              & (5.100)         & (3.167)         \\[1.1em]
ETH Return              &              &              &              & 5.892***        &              &              &              & 26.668***       & 13.233***       \\
                        &              &              &              & (2.909)         &              &              &              & (7.060)         & (4.021)         \\[1.1em]
Gas Price               &              &              &              & 0.144***        &              &              &              & 0.360***        & 0.007           \\
                        &              &              &              & (19.006)        &              &              &              & (37.172)        & (0.835)         \\[1.1em]
%Intercept               & 6.161***     &              &              &                 & 6.753**      &              &              &                 & -13.567***      \\
%                        & (3.611)      &              &              &                 & (1.989)      &              &              &                 & (-19.363)       \\[1.1em]
&  &  &  & &  &  &  & & \\
Observations & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 \\
$\text{R}^2$ & 
0.675 & 0.873 & 0.754 & 0.754 & 
0.671 & 0.836 & 0.958 & 0.889 & 
0.748 \\
Pair FEs & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
\bottomrule
\end{tabular}


==> TAB/TC_reg_no_gas.tex <==
\begin{tabular}{lccccccccc}
\toprule
{}                      & (1)          & (2)          & (3)          & (4)             & (5)          & (6)          & (7)          & (8)             & (9) \\
\midrule
Dep. Variable           & CEX          & CEX          & CEX          & CEX             & DEX          & DEX          & DEX          & DEX             & DEX - CEX       \\
                      & TCs          & TCs          & TCs          & TCs             & TCs          & TCs          & TCs          & TCs             & TCs       \\
&  &  &  &  &  &  &  & & \\
Lagged CEX TC           & 0.954***     &              &              &                 &              &              &              &                 &                 \\
                        & (30.659)     &              &              &                 &              &              &              &                 &                 \\[1.1em]
Lagged DEX TC           &              &              &              &                 &  0.898***    &              &              &                 &                 \\
                        &              &              &              &                 &  (172.515)  &              &              &                 &                 \\[1.1em]
Average CEX TCs         &              & 0.803*       &              &                 &              & -0.585***    &              &                 &                 \\
                        &              & (1.931)      &              &                 &              & (-3.509)     &              &                 &                 \\[1.1em]
Average DEX TCs         &              &              &  -0.158***   &                 &              &              & 1.037***     &                 &                 \\
                        &              &              &  (-3.127)    &                 &              &              & (5.451)      &                 &                 \\[1.1em]
ETH Volume in USD       &              &              &              & -0.023          &              &              &              &  0.449***       & 0.540***        \\
                        &              &              &              & (-0.348)        &              &              &              &  (4.258)        & (3.507)         \\[1.1em]
ETH Return              &              &              &              & -1.586          &              &              &              &  11.647***      & 20.776***       \\
                        &              &              &              & (-0.854)        &              &              &              &  (3.806)        & (6.065)         \\[1.1em]
Gas Price               &              &              &              & 0.004           &              &              &              &  0.011***       & 0.216***        \\
                        &              &              &              & (0.693)         &              &              &              &  (2.625)        & (18.797)        \\[1.1em]
%Intercept               & 6.161***     &              &              &                 & 6.753**      &              &              &                 & -13.567***      \\
%                        & (3.611)      &              &              &                 & (1.989)      &              &              &                 & (-19.363)       \\[1.1em]
&  &  &  & &  &  &  & & \\
Observations & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 & 85,485 \\
R-squared & 
0.933 & 0.381 & 0.272 & 0.257 & 
0.898 & 0.568 & 0.873 & 0.586 &
0.315 \\
Pair FEs & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
\bottomrule
\end{tabular}


==> TAB/TCs_all.tex <==
\begin{tabular}{llrrrrr}
\toprule
Pair &&
ETH-USDC &
ETH-USDT &
ETH-BTC & 
LINK-ETH & 
USDC-USDT \\


\midrule\\[-0.75em]
\multicolumn{7}{c}{\color{Uniswap_color_dark}\textbf{Panel A: Uniswap v2}}\\
\midrule
Exchange Fees &     &   30.000 &   30.000 &  30.000 &   30.000 &    30.000 \\
\midrule
\multirow[c]{2}{*}{B/A Spread} 
        & Mean & 0.774 & 0.925 & 1.032 & 3.030 & 3.466 \\
        %& Median & 0.742 & 0.904 & 1.125 & 3.003 & 3.263 \\
        & Std & 0.159 & 0.207 & 0.376 & 0.970 & 1.326 \\
\midrule
\multirow[c]{2}{*}{Gas Fees} 
        & Mean & 26.072 & 26.072 & 26.072 & 26.069 & 26.072 \\
        %& Median & 21.929 & 21.929 & 21.929 & 21.926 & 21.929 \\
        & Std & 22.906 & 22.906 & 22.906 & 22.906 & 22.906 \\
\midrule
\multirow[c]{2}{*}{Total TC} 
        & Mean & 56.846 & 56.997 & 57.104 & 59.099 & 59.537 \\
        %& Median & 52.723 & 52.937 & 52.831 & 54.672 & 55.292 \\
        & Std & 22.897 & 22.895 & 22.772 & 22.477 & 22.862 \\


\midrule\\[-0.75em]
\multicolumn{7}{c}{\color{Uniswap_v3_color_dark}\textbf{Panel B: Uniswap v3}}\\
\midrule
Exchange Fees &     & 4.529 & 5.211 & 5.378 & 28.341 & 2.030 \\
\midrule
\multirow[c]{2}{*}{B/A Spread} 
    & Mean & 0.457 & 1.816 & 0.474 & 2.689 & 0.007 \\
    %& Median & 0.141 & 0.943 & 0.243 & 1.513 & 0.000 \\
    & Std & 0.862 & 2.751 & 1.237 & 3.189 & 0.105 \\
\midrule
\multirow[c]{2}{*}{Gas Fees} 
    & Mean & 19.630 & 19.630 & 19.630 & 19.630 & 19.630 \\
    %& Median & 7.953 & 7.953 & 7.953 & 7.953 & 7.953 \\
    & Std & 37.529 & 37.529 & 37.529 & 37.529 & 37.529 \\
\midrule
\multirow[c]{2}{*}{Total TC} 
    & Mean & 24.616 & 26.657 & 25.481 & 50.659 & 21.667 \\
    %& Median & 12.981 & 16.126 & 14.125 & 40.340 & 10.333 \\
    & Std & 37.616 & 37.224 & 37.504 & 38.308 & 37.884 \\



\midrule\\[-0.75em]
\multicolumn{7}{c}{\color{Binance_color_dark}\textbf{Panel C: Binance}}\\
\midrule
Exchange Fees     &     &   10.000 &   10.000 &  10.000 &   10.000 &    10.000 \\
\midrule
\multirow[c]{2}{*}{B/A Spread} 
    & Mean & 3.089 & 0.319 & 0.404 & 9.654 & 0.504 \\
    %& Median & 2.948 & 0.159 & 0.147 & 9.109 & 0.500 \\
    & Std & 1.994 & 0.461 & 0.576 & 4.033 & 0.132 \\
\midrule
\multirow[c]{2}{*}{DW Fees} 
    & Mean & 20.370 & 14.854 & 19.226 & 17.474 & 22.542 \\
    %& Median & 18.057 & 12.201 & 15.803 & 14.174 & 17.950 \\
    & Std & 15.910 & 15.269 & 18.331 & 16.349 & 21.801 \\
\midrule
\multirow[c]{2}{*}{Total TC} 
    & Mean & 33.459 & 25.172 & 29.630 & 37.128 & 33.046 \\
    %& Median & 31.198 & 22.538 & 26.648 & 34.384 & 28.453 \\
    & Std & 16.308 & 15.333 & 18.376 & 15.605 & 21.807 \\

\midrule\\[-0.75em]
\multicolumn{7}{c}{\color{Kraken_color_dark}\textbf{Panel D: Kraken}}\\
\midrule
Exchange Fees &     &   26.000 &   26.000 &  26.000 &   26.000 &    26.000 \\
\midrule
\multirow[c]{2}{*}{B/A Spread} 
    & Mean & 4.639 & 2.622 & 2.253 & 19.954 & 1.092 \\
    %& Median & 3.933 & 2.166 & 1.946 & 14.646 & 0.985 \\
    & Std & 5.084 & 2.610 & 1.631 & 15.618 & 1.104 \\
\midrule
\multirow[c]{2}{*}{DW Fees} 
    & Mean & 17.269 & 22.269 & 13.764 & 16.558 & 27.894 \\
    %& Median & 13.462 & 18.465 & 9.865 & 11.365 & 22.289 \\
    & Std & 14.352 & 14.352 & 15.035 & 16.180 & 20.282 \\
\midrule
\multirow[c]{2}{*}{Total TC}              
    & Mean & 47.908 & 50.891 & 42.017 & 62.512 & 54.986 \\
    %& Median & 44.976 & 47.461 & 38.080 & 60.045 & 49.320 \\
    & Std & 15.156 & 14.579 & 14.784 & 19.356 & 20.352 \\


\bottomrule


\end{tabular}




==> TAB/gas_stats.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
 & N & Mean & Std & 1\% & 10\% & 50\% & 90\% & 99\% \\
\midrule
Gas Price (GWEI) & 8,737 & 106.72 & 77.76 & 14.97 & 27.05 & 94.96 & 191.33 & 366.91 \\
Gas cost of a Swap (USD) & 8,737 & 32.68 & 27.58 & 3.54 & 6.60 & 26.50 & 65.48 & 128.96 \\
\bottomrule
\end{tabular}


==> TAB/sum_stats_level_new.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
Level &\qquad      N &\qquad     Mean &\qquad      Std &\qquad       1\% &\qquad      10\% &\qquad      50\% &\qquad      90\% &\qquad      99\% \\
\midrule
Pair-Day & 18,178 & -0.16 & 1.32 & -0.50 & -0.23 & -0.01 & -0.00 & -0.00 \\
Pair & 100 & -0.20 & 0.22 & -0.75 & -0.54 & -0.13 & -0.02 & -0.00 \\
Day & 352 & -0.20 & 0.37 & -0.69 & -0.38 & -0.11 & -0.04 & -0.03 \\
\bottomrule
\end{tabular}

